A Wendelstein-7X Profile Database for Informed Transport Studies

To advance the development of future fusion devices beyond Wendelstein 7-X (W7-X), a robust understanding of energy confinement time scaling is crucial. Universal temperature and density profile shapes are theoretically anticipated through a comparison of the empirical ISS04 confinement time scaling with predictions based on Gyro-Bohm heat flux scaling. This thesis investigates the presence of these universalities in W7-X experimental profiles and subsequently tests existing confinement time scalings against this data. Experimental profiles are obtained from Thomson scattering diagnostics. Gradient length scales, defined as the radial derivative of the logarithmic quantity of the investigated profiles, are extracted from these profiles through fitting procedures. These scales serve as boundary conditions for subsequent gyrokinetic flux-tube simulations using the GX code. The simulated heat fluxes are then employed to reconstruct profiles by solving the power balance equation and density evolution. A comparison of these reconstructed profiles with the averaged experimental profiles reveals that the predicted density profiles are steeper than those measured in the reference dataset. To investigate this discrepancy, additional discharges exhibiting more peaked density profiles, including both high-performance and low-power plasmas, are examined. Furthermore, the ratio of experimental temperature and density scale lengths is incorporated as an input into the simulations, and the resulting simulated heat fluxes are evaluated. Discrepancies between the simulated and measured profiles are discussed, with potential explanations encompassing particle sources and neoclassical transport mechanisms. This comprehensive approach aims to deepen our understanding of the critical role of profile shape and transport mechanisms in plasma confinement.

==> acronyms.tex <==
\makeglossaries
\newacronym{gcd}{GCD}{Greatest Common Divisor}

\newacronym{W7-X}{W7-X}{Wendelstein 7-X}
\newacronym{MHD}{MHD}{Magnetohydrodynamics}
\newacronym{VMEC}{VMEC}{Variational Moments Equilibrium Code}
\newacronym{ECRH}{ECRH}{Electron Resonance Cyclotron Heating}
\newacronym{NBI}{NBI}{Neutral Beam Injection}
\newacronym{TS}{TS}{Thomson Scattering}

\newacronym{LCFS}{LCFS}{Last Closed Flux Surface}

\newacronym{ODEs}{ODEs}{Ordinary Differential Equations}

\newacronym{ITG}{ITG}{Ion Temperature Gradient}
\newacronym{ETG}{ETG}{Electron Temperature Gradient}
\newacronym{TEM}{TEM}{Trapped Electron Mode}

\newacronym{ML}{ML}{Machine Learning}
\newacronym{CG}{CG}{Critical Gradient}

\newacronym{ISS04}{ISS04}{International Stellarator Scaling 2004}

\newacronym{XICS}{XICS}{X-ray Imaging Crystal Spectrometer}
\newacronym{CXRS}{CXRS}{Charge Exchange Recombination Spectroscopy}


\newacronym{GB}{GB}{Gyro-Bohm}


==> lib/kthcolors.tex <==
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:
% KTH colors for LaTeX documents
%
% Started from kthcolors by:
% Riccardo Sven Risuleo
% 2016-09-06 11:05:40
%
% from https://github.com/KTH-AC/kthcolors
%
% Adapted using the colors from "Graphic Profile Manual KTH" version 180604
% (i.e.. 2018-06-04) 
% see https://intra.kth.se/en/administration/kommunikation/grafiskprofil/kth-s-grafiska-profil-1.844676
% 
% G. Q. Maguire Jr.
% 2021-07-05
%

%\NeedsTexFormat{LaTeX2e}[1994/06/01]
%\ProvidesPackage{kthcolors}[2021/07/85 v3 Latex package with official KTH colors]

\RequirePackage{xcolor}
%% Primary colors
%% As of the new manual, there is only 1 primary color; but with three 
\definecolor{kth-blue}{RGB/cmyk}{25,84,166/0.849,0.494,0,0.349}
\colorlet{kth-blue80}{kth-blue!80!}
\colorlet{kth-blue40}{kth-blue!40!}

% these are no longer used as of 2018-06-04
%\definecolor{kth-red}{RGB/cmyk}{157,16,45/0,0.898,0.713,0.384}
%\definecolor{kth-green}{RGB/cmyk}{98,146,46/0.329,0,0.685,0.427}

%% Secondary colors
\definecolor{kth-lightblue}{RGB/cmyk}{36,160,216/0.833,0.259,0,0.153}
\colorlet{kth-lightblue80}{kth-lightblue!80!}
\colorlet{kth-lightblue40}{kth-lightblue!40!}

%\definecolor{kth-lightred}{RGB/cmyk}{228,54,62/0,0.763,0.728,0.106}
\definecolor{kth-lightred}{RGB}{216,84,151}
\colorlet{kth-lightred80}{kth-lightred!80!}
\colorlet{kth-lightred40}{kth-lightred!40!}

\definecolor{kth-lightgreen}{RGB/cmyk}{176,201,43/0.124,0,0.786,0.212} % olive
\colorlet{kth-lightgreen80}{kth-lightgreen!80!}
\colorlet{kth-lightgreen40}{kth-lightgreen!40!}

% Cool Gray 9C
%\definecolor{kth-coolgray}{RGB}{101,101,108}

% Cool Gray 10 suggested by Martin Krzywinski (see http://mkweb.bcgsc.ca/colorblind) 
\definecolor{kth-coolgray}{RGB}{99,102,106}
\colorlet{kth-coolgray80}{kth-coolgray!80!}
\colorlet{kth-coolgray40}{kth-coolgray!40!}

% Tertiary colors (yet more colors)
% All of these are no longer used
%\definecolor{kth-pink}{RGB/cmyk}{216,84,151/10,0.611,0.301,0.153}
%\definecolor{kth-yellow}{RGB/cmyk}{250,185,25/0,0.26,0.9,0.0196}
%\definecolor{kth-darkgray}{RGB/cmyk}{101,101,108/0.0648,0.0648,0,0.576}
%\definecolor{kth-middlegray}{RGB/cmyk}{189,188,188/0,0.00529,0.00529,0.259}
%\definecolor{kth-lightgray}{RGB/cmyk}{227,229,227/0.00873,0,0.00873,0.102}

%\DeclareOption{gray}{\colorlet{gray}{kth-darkgray}}

% These versions are designed to meet accessability requirements for digital media
% Note that the palette is more limited than for the print version of the colors
\ifdigitaloutput
    % primary color
    \definecolor{kth-blue}{HTML}{1954A6} % Deep sea
    \definecolor{kth-blue80}{HTML}{5E87C0}

    % Secondary colors
    \definecolor{kth-lightblue}{HTML}{2191C4} % Stratosphere
    \definecolor{kth-lightred}{HTML}{D02F80} % Fluorescence
    \definecolor{kth-lightred80}{HTML}{D95599}
    \definecolor{kth-lightgreen}{HTML}{62922E} % Front-lawn
    \definecolor{kth-coolgray}{HTML}{65656C} % Office
    \definecolor{kth-coolgray80}{HTML}{848489}
\fi


